Double Thompson Sampling for Dueling Bandits

In this paper, we propose a Double Thompson Sampling (D-TS) algorithm for dueling bandit problems. As indicated by its name, D-TS selects both the first and the second candidates according to Thompson Sampling. Specifically, D-TS maintains a posterior distribution for the preference matrix, and chooses the pair of arms for comparison by sampling twice from the posterior distribution. This simple algorithm applies to general Copeland dueling bandits, including Condorcet dueling bandits as its special case. For general Copeland dueling bandits, we show that D-TS achieves $O(K^2 \log T)$ regret. For Condorcet dueling bandits, we further simplify the D-TS algorithm and show that the simplified D-TS algorithm achieves $O(K \log T + K^2 \log \log T)$ regret. Simulation results based on both synthetic and real-world data demonstrate the efficiency of the proposed D-TS algorithm.

==> app_regret_condorcet.tex <==
\section{Regret Analysis in Condorcet Dueling Bandits} \label{app:regret_condorcet}

In this appendix, we discuss the proof of Theorem~\ref{thm:regret_condorcet}. We can show an $O(K^2 \log T)$ regret for \sdts similarly to  \cite{Agrawal2013AISTATS:TS2} and that for general Copeland dueling bandits, as stated in Proposition~\ref{thm:regret_condorcet_weak}. The complete proof for Proposition~\ref{thm:regret_condorcet_weak} is omitted here due to the similarity, and we only discuss the analysis for the part we need to refine.

To refine the bound to $O(K\log T + K^2 \log T)$, we only need to refine the third term in Eq.~\eqref{eq:regret_condorcet_weak}, which is the bound for the number of comparisons between $i\notin \mathcal{C}^*$ and $j \neq j_i^*$. Note that under \sdts, when fixing the first candidate as $a_{t}^{(1)} = i$, we compare $i$ with all $j$ to find the best arm $j_i^*$. Thus, each arm $j$ is competing with $j^*_i$, rather than $i$. Thus, different from the analysis for  the original D-TS,
the proof should be modified accordingly, which becomes more similar to the analysis of Thompson Sampling for traditional MAB \cite{Agrawal2013AISTATS:TS2}.

Similar to  \cite{Agrawal2013AISTATS:TS2}, for $j \neq j^*_i$,  we choose two numbers $x_{ji}$, $y_{ji}$, such that $p_{ji} < x_{ji} < y_{ji} < p_i^*=\max_j p_{ji}$. Redefine the events as follows:

\begin{equation}
\mathcal{E}^{\bar{p}}_{ji}(t) = \{\bar{p}_{ji}(t) < x_{ji}\},
\end{equation}
and
\begin{equation}
\mathcal{E}^{\theta}_{ji}(t) = \{\theta^{(2)}_{ji}(t) < y_{ji} \}.
\end{equation}

To further refine the bound to $O(K\log T + K^2 \log T)$, we only need to refine the proof of Lemma~4 in \cite{Agrawal2013AISTATS:TS2},
because other components are bounded by $O(1)$.
%(which is implied as \eqref{eq:p_leq0p5_sec_term} for the original D-TS in Copeland dueling bandits).
To show how to refine this proof, we recall the key step in the proof of Lemma~4 in \cite{Agrawal2013AISTATS:TS2} , which bounds the expected number of steps when $(i,j)$ ($j \neq j_i^*$) are compared while $\bar{p}_{ji} < x_{ji}$ and $\theta^{(2)}_{ji}(t) \geq y_{ji}$:
\begin{eqnarray}
&&\sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t)\} \nonumber \\
&\leq& \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), N_{ij}(t-1) \leq L_{ji}(T)\}  \nonumber \\
&& +  \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), N_{ij}(t-1) >   L_{ji}(T)\} \nonumber \\
&\leq & L_{ji} (T) + \sum_{t = 1}^T \frac{1}{T} \nonumber \\
&=& \frac{\log T}{D(x_{ji}|| y_{ji})} + 1,
\end{eqnarray}
where $L_{ji} (T)$ is defined as  $L_{ji} (T) = \frac{\log T}{D(x_{ji}|| y_{ji})}$ (slightly different from that in the original D-TS, because in that case $j$ is competing with $i$ with $p_{ii} = 1/2$ and we can just let $y_{ji} = 1/2$.).

To further reduce the regret, we consider the distribution of $N_{i}^{(1)}(T)$, which is the number of steps that arm $i$ is chosen as the first candidate, i.e., $N_{i}^{(1)}(T) = \sum_{t=1}^T \mathbbm{1}(a_t^{(1)} = i)$ .
For $\alpha > 0.5$, let
\begin{eqnarray}
 L^{\alpha}_{ji}(n) = \frac{(1+2\alpha) \log n} {D(x_{ji}|| y_{ji})}.
\end{eqnarray}
Then,
\begin{eqnarray}
&&\sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t)\} \nonumber \\
&=& \sum_{n=0}^T \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), N_{ij}(t-1) \leq L^{\alpha}_{ji}(n), N_{i}^{(1)}(T) = n\}  \nonumber \\
&& + \sum_{n=0}^T \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), N_{ij}(t-1) >   L^{\alpha}_{ji}(n), N_{i}^{(1)}(T) = n\} .\end{eqnarray}
We can bound the first term as:
\begin{eqnarray}
&&  \sum_{n = 0}^{T} \sum_{t = 1}^T  \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), {N_{ij}(t-1) \leq L^{\alpha}_{ji}(n), N_{i}^{(1)}(T) = n}\} \nonumber \\
&=&  \sum_{n = 0}^{T}\sum_{t = 1}^T  \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), {N_{ij}(t-1) \leq L^{\alpha}_{ji}(n) |  N_{i}^{(1)}(T) = n}\} \mathbb{P}\{ N_{i}^{(1)}(T) = n\} \nonumber \\
&\overset{(a)}{\leq} & \sum_{n = 0}^{T} L^{\alpha}_{ji}(n)  \mathbb{P}\{ N_{i}^{(1)}(T) = n\}  \nonumber \\
&= & \frac{\mathbb{E}[(1 + 2\alpha)\log N_{i}^{(1)}(T)]}{D(x_{ji}|| y_{ji})} \overset{(b)}{\leq} \frac{(1+ 2\alpha)\log \mathbb{E}[ N_{i}^{(1)}(T)]}{D(x_{ji}|| y_{ji})},
\end{eqnarray}
where $(b)$ holds due to the concavity of the $\log(\cdot)$ function, and $(a)$ holds because, similar to the discussion in Appendix~\ref{app:proof_cmp_bounds_larger_0p5}, we have
\begin{eqnarray}
&&  \sum_{t = 1}^T  \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), {N_{ij}(t-1) \leq L^{\alpha}_{ji}(n) \big|  N_{i}^{(1)}(T) = n}\} \nonumber \\
&= & \sum_{t = 1}^T \mathbb{E}\bigg[\mathbbm{1}\big((a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), {N_{ij}(t-1) \leq L^{\alpha}_{ji}(n) \big) \big| N_{i}^{(1)}(T) = n}\bigg] \nonumber \\
&\leq & \mathbb{E}\bigg[\sum_{t = 1}^T \mathbbm{1}\big((a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), {N_{ij}(t-1) \leq L^{\alpha}_{ji}(n) \big) \big| N_{i}^{(1)}(T) = n}\bigg] \nonumber \\
&= & L^{\alpha}_{ji}(n). \nonumber
\end{eqnarray}

For any $\epsilon > 0$, choosing appropriate $x_{ji}$ and $y_{ji}$ such that $D(x_{ji}|| y_{ji}) = D(p_{ji}|| p^*_i)/(1+\epsilon)^2$, similar to \cite{Agrawal2013AISTATS:TS2}, we have
 \begin{eqnarray} \label{eq:refine_regret_part1}
&&  \sum_{n = 0}^{T} \sum_{t = 1}^T  \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), {N_{ij}(t-1) \leq L^{\alpha}_{ji}(n), N_{i}^{(1)}(T) = n}\} \nonumber \\
&\leq&  \frac{(1+ 2\alpha)(1+\epsilon)^2\big(\log \log T + O(\log K)\big)}{D(p_{ji}|| p^*_i)}.
\end{eqnarray}


For the second term, different from the proof for the $O(K^2\log T)$ regret, we analyze the probability at the time-slot where $i$ is selected as the first candidate. Specifically, let $\tau^{(i)}_m$ be the time-slot index where $i$ is  chosen as the first candidate for the $m$-th time, and let $\tau^{(i)}_0 = 0$. Then,
\begin{eqnarray}
&& \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t),N_{ij}(t-1) > L^{\alpha}_{ji}(n), N_i^{(1)}(T) = n \}  \nonumber\\
& = & \mathbb{E}\bigg[\sum_{t = 1}^T \mathbbm{1}\big((a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t),N_{ij}(t-1) > L^{\alpha}_{ji}(n), N_i^{(1)}(T) = n \big)\bigg]  \nonumber\\
&\leq & \sum_{m = 0}^{n-1} \mathbb{E}\bigg[\sum_{t = \tau^{(i)}_m + 1}^{\tau^{(i)}_{m+1}} \mathbbm{1}\big((a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t),N_{ij}(t-1) > L^{\alpha}_{ji}(n) \big)\bigg] \nonumber \\
& \overset{(c)}{\leq} & \sum_{m = 0}^{n-1} \mathbb{E}\big[\mathbbm{1}((a_{\tau^{(i)}_{m+1}}^{(1)}, a_{\tau^{(i)}_{m+1}}^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(\tau^{(i)}_{m+1}), \urcorner \mathcal{E}^{\theta}_{ji}(\tau^{(i)}_{m+1}), N_{ij}(\tau^{(i)}_{m+1}-1) > L^{\alpha}_{ji}(n))\big] \nonumber\\
& \leq &  \sum_{m = 0}^{n-1} \mathbb{P}\{  \mathcal{E}^{\bar{p}}_{ji}(\tau^{(i)}_{m+1}), \urcorner \mathcal{E}^{\theta}_{ji}(\tau^{(i)}_{m+1}),N_{ij}(\tau^{(i)}_{m+1}-1) > L^{\alpha}_{ji}(n)\big\} \nonumber\\
& \overset{(d)}{\leq} &  n \cdot \frac{1}{n^{1+2\alpha}} = \frac{1}{n^{2\alpha}}, \nonumber
\end{eqnarray}
where $(c)$ holds because $a_t^{(1)} = i$ could only happen at $t = \tau^{(i)}_{m+1}$; $(d)$ is true because, given $N_{ij}(\tau^{(i)}_{m+1}-1) > L^{\alpha}_{ji}(n)$, the events  $\mathcal{E}^{\bar{p}}_{ji}(t)$ and $\mathcal{E}^{\theta}_{ji}(t)$ are independent of $t = \tau^{(i)}_{m+1}$, and thus the probability can be bounded according to the concentration property of Thompson samples (in the proof of Lemma~3 in \cite{Agrawal2013AISTATS:TS2}):
\begin{equation}
\mathbb{P}\{\mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t)|N_{ij}(t-1) > L^{\alpha}_{ji}(n)\} \leq e^{-L^{\alpha}_{ji}(n) D(x_{ji}||y_{ji})} = \frac{1}{n^{1 + 2\alpha}}. \nonumber 
\end{equation}

Thus, \label{eq:refine_regret_part2}
\begin{eqnarray}
&&\sum_{n = 0}^{T} \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t), N_{ij}(t-1) > L^{\alpha}_{ji}(n), N_{i}^{(1)}(T) = n\}  \nonumber \\
&\leq & \sum_{n = 0}^{T} \frac{1}{n^{2\alpha}} =O(1) \nonumber\\
\end{eqnarray}

For any $i \notin C^*$, and $j \neq j_i^*$, using the $O(1)$ bounds for the $\{\mathcal{E}^{\bar{p}}_{ji}(t), \mathcal{E}^{\theta}_{ji}(t) \}$ and $\mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t)$ cases, we have
\begin{eqnarray}
\mathbb{E}[N_{ij}^{(1)}(T)] &=&  \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t)\} \nonumber \\
&& + \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \mathcal{E}^{\theta}_{ji}(t)\} \nonumber \\
&& + \sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \urcorner\mathcal{E}^{\bar{p}}_{ji}(t)\} \nonumber \\
&=&\sum_{t = 1}^T \mathbb{P}\{(a_t^{(1)}, a_t^{(2)}) = (i,j),  \mathcal{E}^{\bar{p}}_{ji}(t), \urcorner \mathcal{E}^{\theta}_{ji}(t)\} + O(1) \nonumber \\
&\leq& \frac{(1+ 2\alpha)(1+\epsilon)^2\big(\log \log T + O(\log K)\big)}{D(p_{ji}|| p^*_i)} + O(1).
\end{eqnarray}

The conclusion of the theorem follows by replacing the third term in Eq.~\eqref{eq:regret_condorcet_weak} according to the above inequation. 


==> intro_backup_beforeLiu.tex <==
\section{Introduction} \label{sec:intro}
\aftersec
The dueling bandit problem \cite{Yue2012JCSS:DuelingBandits} is a variant of the classical multi-armed bandit (MAB) problem, where the feedback comes in the format of pairwise comparison. This model has attracted much attention as it can be applied in systems such as information retrieval (IR) \cite{Yue2009ICML:DuelingBandits,Zoghi2014WSDM:RCS}, where user preferences are  easier to obtain and typically more stable.
Most earlier work \cite{Yue2012JCSS:DuelingBandits,Zoghi2014ICML:RUCB,Komiyama2015COLT:DB} focuses on Condorcet dueling bandits, where there exists an arm, referred to as the Condorcet winner, that beats all other arms.
%However, the existence of Condorcet winner is not guaranteed in practice.
Recent work \cite{Zoghi2015NIPS:CDB,Komiyama2016ICML:CWRMED} turns to more general and practical settings with a Copeland winner(s), which is the arm (or arms) that beats the most other arms.
%A recent work \cite{Zoghi2015NIPS:CDB} studies general Copeland dueling bandits and proposes a Copeland Confidence Bound (CCB) algorithm that achieves logarithmic regret. A recently accepted paper \cite{Komiyama2016ICML:CWRMED} reveals a lower regret bound for Copeland dueling bandits, and proposes an optimal algorithm CW-RMED and its computationally efficient version ECW-RMED.
Most existing algorithms are mainly generalized from traditional MAB algorithms along two lines, e.g., RUCB \cite{Zoghi2014ICML:RUCB} and CCB \cite{Zoghi2015NIPS:CDB} are UCB (Upper Confidence Bound)-type algorithms, while RMED \cite{Komiyama2015COLT:DB} and CW-RMED/ECW-RMED \cite{Komiyama2016ICML:CWRMED} are MED (Minimum Empirical Divergence)-type algorithms.

An alternative efficient solution to traditional MAB is Thompson Sampling \cite{Thompson1933FirstMAB}. The basic idea of Thompson Sampling is simply choosing the optimal action that maximizes the expected reward according to the randomly drawn belief.
%assuming certain prior distribution for the system parameters, the algorithm maintains the posterior distribution for these parameters and takes the best action according to samples drawn from the posterior distribution; the feedback of the system under the taken action is then used to update the posterior distribution.
Thompson Sampling has been successfully applied in traditional MAB \cite{Chapelle2011NIPS:TS,Agrawal2012COLT:TS,Komiyama2015ICML:MP_TS,Qin&Liu2015IJCAI:TS} and other online learning problems \cite{Gopalan2014ICML:TS,Gopalan2015COLT:TSMDP}.
In particular, empirical studies  in \cite{Chapelle2011NIPS:TS} have shown that this simple framework performs better than or close to other types of algorithms in practice, and \cite{Agrawal2012COLT:TS,Agrawal2013AISTATS:TS2} have obtained the theoretical bounds for Thompson Sampling in traditional MAB by analyzing the concentration property of Thompson samples.

Inspired by the success of Thompson Sampling in traditional MAB and other online learning problems, a natural question  is  whether it can be applied to dueling bandits and how.
Unfortunately, the standard framework of Thompson Sampling may not directly apply to dueling bandits because not all comparisons provide information about the system statistics. Specifically, a good learning algorithm for dueling bandits is expected to end up with comparing the winner against itself  \footnote{In practice, when comparing an arm against itself, one does not need to conduct an actual comparison but just implement this arm directly.}.  However, comparing one arm against itself does not provide any system statistical information and cannot be used to update the posterior distribution.
%This is different from traditional MAB, where pulling suboptimal arms accumulates knowledge of their distributions so that the algorithm can gradually gets out of the suboptimal actions.
Therefore, the Thompson Sampling algorithm needs to be adjusted here so that: 1) comparing the winners against themselves is allowed, but, 2) trapping in comparing suboptimal arm/arms against itself/themselves is avoided.

In this paper, we propose a Double Thompson Sampling (D-TS) algorithm for dueling bandits, including both Condorcet dueling bandits and general Copeland dueling bandits. As indicated by its name,  D-TS typically selects both the first and the second candidates according to samples independently drawn from the posterior distributions.
Confidence bound methods are also leveraged to eliminate the likely non-winner arms, so that trapping in suboptimal comparisons is avoided.
%We resort to RUCB because the samples drawn from the posterior distribution are random and cannot be used to judge an arm of being a winner or not with a given confidence level, although they drop in the confidence intervals with high probability.
Compared to preliminary trial, RCS \cite{Zoghi2014WSDM:RCS}, in Condorcet dueling bandits, where the first candidate is selected by Thompson Sampling but the second candidate is selected by RUCB, our D-TS algorithm has both practical and theoretical advantages.

First of all, the double sampling structure of D-TS fits better to the nature of dueling bandits. Launching another round of independent sampling provides us the opportunity to select the same arm as the first candidate and thus to compare the winners against themselves. As expected, this double sampling structure leads to more full utilization of Thompson Sampling than RCS, and significantly reduces the regret. Moreover, this simple framework applies to general Copeland dueling bandits and achieves much better performance than existing algorithms such as CCB \cite{Zoghi2015NIPS:CDB}.
%One may suggest treating each pair of arms as a complex action and apply the simple framework of Thompson Sampling in \cite{Gopalan2014ICML:TS}. However, as discussed previously, not all comparisons provide information and it is unclear how to select the pair according to the samples, especially for general Copeland dueling bandits.
%Without special treatment, using the simple framework may get stuck on comparing non-winners.

Second, by leveraging the properties of this double sampling structure, we are able to obtain theoretical bounds for D-TS.  As noted in traditional MAB literature \cite{Agrawal2012COLT:TS,Agrawal2013AISTATS:TS2}, theoretical analysis of Thompson Sampling is usually more difficult than UCB-type algorithms.
The analysis in dueling bandits is even more difficult because the selection of arms involves more factors and the two selected arms may be correlated.
%For example, an arm that is selected as the first candidate may also have a higher probability (than that in traditional MAB) to be chosen as the second candidate.
Our D-TS algorithm can address this issue because the two sets of samples are drawn independently and their distributions are captured by historic comparison results. Thus, when fixing the first candidate as a specific arm, the comparison between it and all other arms is similar to traditional MAB and hence the ideas for traditional MAB can be borrowed.  By investigating the properties of Thompson Sampling and confidence bounds, we show that  D-TS achieves $O(K^2 \log T)$ regret
for a general $K$-armed Copeland dueling bandit. More interestingly, the property that the sample distribution only depends on historic comparing results (but not $t$)  enables us to refine the regret by a \emph{back substitution} argument, where we show that D-TS achieves $O(K \log T + K^2 \log \log T)$ in many practical scenarios and Condorcet dueling bandits.
%we have shown that we can bound the number of time-slots when a non-winner arm is chosen as the first candidate  by $O(\log T)$. Then by viewing the comparison between it and all other arms as a traditional MAB, we can bound the number of comparison between this arm and the suboptimal arms (that is beaten by it) is further reduced to $O(\log \log T)$ due to the concavity of the logarithmic function. Then the total regret is reduced to $O(K L_C \log T + K^2 \log \log T)$ regret, where $L_C$ is the number of arms that beats the Copeland winners.

Based on the analysis, we refine the tie-breaking criterion in D-TS and propose its enhancement called D-TS$^+$. D-TS$^+$ achieves the same theoretical regret bound as D-TS, but performs better especially when there are multiple winners.

% Furthermore, this algorithm applies to many dueling bandit problems with different definitions of winner, including both  the Condorcet winner \cite{Yue2012JCSS:DuelingBandits,Yue2009ICML:DuelingBandits}  and the Copeland winner \cite{Zoghi2015NIPS:CDB}.

In summary, the main contributions of this paper are as follows:
\begin{itemize}
\item We propose a D-TS algorithm and its enhancement D-TS$^+$ for general Copeland dueling bandits. The double sampling structure fits to the nature of dueling bandits and leads to full utilization of Thompson Sampling, which significantly reduces the regret.
    %Our study also demonstrates how to deal with the unique difficulties when using Thompson Sampling in dueling bandits, e.g., using RUCB/RLCB-based elimination to avoid trapping in suboptimal comparisons.
\item We obtain theoretical regret bounds for D-TS. For general Copeland dueling bandits, we show that the proposed D-TS and D-TS$^+$ algorithms achieve $O(K^2 \log T)$ regret. In Condorcet dueling bandits and most practical scenarios, we further refine the regret bound to $O(K \log T + K^2 \log \log T)$ by a back substitution argument.
\item We evaluate the D-TS and D-TS$^+$ algorithms through experiments based on both synthetic and real-world data. The experiment results demonstrate the effectiveness of this double sampling structure.
\end{itemize}
\aftersec
\aftersec
\section{Related Work}
\aftersec
Many algorithms have been proposed to solve dueling bandits since \cite{Yue2012JCSS:DuelingBandits}. Earlier algorithms such as IF \cite{Yue2012JCSS:DuelingBandits}, BTM \cite{Yue2011ICML:BTM}, and SAVAGE \cite{Urvoy2013ICML:SAVAGE} belong to the type of ``explore-then-exploit'' algorithms and only apply to  finite-horizon settings. For infinite horizon settings, recent work has generalized the traditional UCB and MED algorithms to dueling bandits. For example, RUCB \cite{Zoghi2014ICML:RUCB} and CCB \cite{Zoghi2015NIPS:CDB} are generalizations of UCB for Condorcet and general Copeland dueling bandits, respectively. \cite{Ailon2014ICML:UBDB} reduces dueling bandits to traditional MAB, which is then solved by their proposed UCB-type algorithms, MutiSBM and Sparring.
%\cite{Zoghi2014ICML:RUCB} extends the classic Upper Confidence Bound (UCB) method \cite{Auer2002ML:UCB} to dueling bandits and proposes a Relative Upper Confidence Bound (RUCB) algorithm that achieves $O(K \log T)$ regret in $K$-armed dueling bandits. The more recent work  \cite{Komiyama2015COLT:DB} proposes  a Relative Minimum Empirical Divergence (RMED) algorithm, which is shown to be optimal in the sense of both the asymptotic order $O(K \log T)$ and the constant coefficient, under the Condorcet assumption.
%These algorithms are proposed for Condorcet dueling bandits, while the existence of a Condorcet winner is not guaranteed in practice \cite{Urvoy2013ICML:SAVAGE,Zoghi2015NIPS:CDB}.
On the other hand, \cite{Komiyama2015COLT:DB} and the recently accepted work \cite{Komiyama2016ICML:CWRMED} extend the traditional MED algorithm to dueling bandits, where they present the lower bound of the regret and propose the corresponding optimal algorithms, including RMED \cite{Komiyama2015COLT:DB} for Condorcet dueling bandits, CW-RMED  and its computationally efficient version ECW-RMED \cite{Komiyama2016ICML:CWRMED} for general Copeland dueling bandits. Different from these existing work, we study algorithms for dueling bandits from the perspective of Thompson Sampling, which is expected to achieve lower regret.
%Another definition of winner is the Borda winner, which is that arm that has the highest total probability of beating other arms. Because Borda dueling bandits can be reduced to the traditional MAB problem \cite{Urvoy2013ICML:SAVAGE,Zoghi2014ICML:RUCB}, only a few researchers study this problem with special structures, such as sparseness \cite{Jamieson2015AISTAT:SDB}. By treating each pair as an action, the SAVAGE algorithm \cite{Urvoy2013ICML:SAVAGE} applies to dueling bandits with all the above three definitions of winners, but it is an ``explore-then-exploit'' algorithm and exploring all pairs of arms may result in a large regret.


Dating back to 1933, Thompson Sampling \cite{Thompson1933FirstMAB} is one of the earliest algorithms for ``exploration-and-exploitation'' tradeoff and has been widely applied in traditional MAB.
%The Thompson Sampling algorithm makes decisions according to random samples drawn from the posterior distribution and updates the posterior distribution according to the system feedbacks under the taken action.
Empirical studies have shown that Thompson Sampling achieves performance better than or close to that of  UCB-type algorithms in practice \cite{Chapelle2011NIPS:TS}. However, theoretical analysis of Thompson Sampling is much more difficult  and a lot of efforts have been made to bound the regret theoretically.  In particular, \cite{Agrawal2012COLT:TS} proposes a logarithmic bound for the standard frequentist expected regret, whose constant factor is further improved in \cite{Agrawal2013AISTATS:TS2}.  On the other hand, through information-theoretic analysis, \cite{Russo2014TR:TS,Russo2014MOR:TS} derive the bounds for its Bayesian expected regret. Nowadays, Thompson Sampling becomes a popular method that has been applied in many variants of MAB \cite{Komiyama2015ICML:MP_TS,Qin&Liu2015IJCAI:TS,Gopalan2014ICML:TS} and other more complex problems, e.g., \cite{Gopalan2015COLT:TSMDP}.

Thompson Sampling has been preliminarily studied for dueling bandits. A rough idea was first discussed at a workshop \cite{Welsh2012LSOLDM:TS}, where the presenter suggests viewing the (normalized) preference matrix as the transition probability matrix for a Markov chain and selecting the arms by sampling from the posterior stationary distribution. Neither the formal description of this idea nor its theoretical analysis is available.
A recent work \cite{Zoghi2014WSDM:RCS} proposes a Relative Confidence Sampling (RCS) algorithm that combines Thompson Sampling with RUCB \cite{Zoghi2014ICML:RUCB}  for Condorcet dueling bandits. Under RCS, the first arm is selected by Thompson Sampling while the second arm is selected according to their RUCB. Empirical studies demonstrate the performance improvement by using RCS in practice, but no theoretical bounds on the regret are provided.



==> intro_backup_beforeLiu0519.tex <==
\section{Introduction} \label{sec:intro}
\aftersec
The dueling bandit problem \cite{Yue2012JCSS:DuelingBandits} is a variant of the classical multi-armed bandit (MAB) problem, where the feedback comes in the format of pairwise comparison. This model has attracted much attention as it can be applied in systems such as information retrieval (IR) \cite{Yue2009ICML:DuelingBandits,Zoghi2014WSDM:RCS}, where user preferences are  easier to obtain and typically more stable.
Most earlier work \cite{Yue2012JCSS:DuelingBandits,Zoghi2014ICML:RUCB,Komiyama2015COLT:DB} focuses on Condorcet dueling bandits, where there exists an arm, referred to as the Condorcet winner, that beats all other arms.
%However, the existence of Condorcet winner is not guaranteed in practice.
Recent work \cite{Zoghi2015NIPS:CDB,Komiyama2016ICML:CWRMED} turns to more general and practical settings with a Copeland winner(s), which is the arm (or arms) that beats the most other arms.
%A recent work \cite{Zoghi2015NIPS:CDB} studies general Copeland dueling bandits and proposes a Copeland Confidence Bound (CCB) algorithm that achieves logarithmic regret. A recently accepted paper \cite{Komiyama2016ICML:CWRMED} reveals a lower regret bound for Copeland dueling bandits, and proposes an optimal algorithm CW-RMED and its computationally efficient version ECW-RMED.
Most existing algorithms are mainly generalized from traditional MAB algorithms along two lines: 1)  UCB (Upper Confidence Bound)-type algorithms, such as RUCB \cite{Zoghi2014ICML:RUCB} and CCB \cite{Zoghi2015NIPS:CDB}; and 2) MED (Minimum Empirical Divergence)-type algorithms, such as RMED \cite{Komiyama2015COLT:DB} and CW-RMED/ECW-RMED \cite{Komiyama2016ICML:CWRMED}.

In traditional MAB, an alternative effective solution is
Thompson Sampling  (TS) \cite{Thompson1933FirstMAB}. Its principle is to choose the optimal action that maximizes the expected reward according to the randomly drawn belief.
%assuming certain prior distribution for the system parameters, the algorithm maintains the posterior distribution for these parameters and takes the best action according to samples drawn from the posterior distribution; the feedback of the system under the taken action is then used to update the posterior distribution.
Thompson Sampling has been successfully applied in traditional MAB \cite{Chapelle2011NIPS:TS,Agrawal2012COLT:TS,Komiyama2015ICML:MP_TS,Qin&Liu2015IJCAI:TS} and other online learning problems \cite{Gopalan2014ICML:TS,Gopalan2015COLT:TSMDP}.
\blue{In particular, empirical studies  in \cite{Chapelle2011NIPS:TS} have shown that this simple framework performs better than other algorithms and is robust to delayed feedback due to its randomization policy.}
% and \cite{Agrawal2012COLT:TS,Agrawal2013AISTATS:TS2} have obtained the theoretical bounds for Thompson Sampling in traditional MAB by analyzing the concentration property of Thompson samples.
%\xl{more advantages of TS here?, e.g., easy to implement and robustness to delayed feedback.}

In the wake of the success of Thompson Sampling (TS) in these online learning problems, a natural question  is  whether  and how TS can be applied to dueling bandits to further improve the performance. However, it is challenging to apply the standard TS framework to dueling bandits because not all comparisons provide information about the system statistics. Specifically, a good learning algorithm for dueling bandits will eventually compare the winner against itself  \footnote{In practice, when comparing an arm against itself, one does not need to conduct an actual comparison but just implement this arm directly.}.  However, comparing one arm against itself does not provide any system statistical information that is critical in TS to update the posterior distribution.
%This is different from traditional MAB, where pulling suboptimal arms accumulates knowledge of their distributions so that the algorithm can gradually gets out of the suboptimal actions.
Therefore, TS needs to be adjusted here so that 1) comparing the winners against themselves is allowed, but, 2) trapping in comparing suboptimal arm/arms against itself/themselves is avoided.

In this paper, we propose a Double Thompson Sampling (D-TS) algorithm for dueling bandits, including both Condorcet dueling bandits and general Copeland dueling bandits. As its name suggests,  D-TS typically selects both the first and the second candidates according to samples independently drawn from the posterior distributions.  D-TS also utilizes the idea of
confidence bounds to eliminate the likely non-winner arms, so that trapping in suboptimal comparisons is avoided.
%We resort to RUCB because the samples drawn from the posterior distribution are random and cannot be used to judge an arm of being a winner or not with a given confidence level, although they drop in the confidence intervals with high probability.
%Compared to  RCS \cite{Zoghi2014WSDM:RCS}, proposed for Condorcet dueling bandits, where the first candidate is selected by Thompson Sampling but the second candidate is selected by RUCB, our D-TS algorithm has both practical and theoretical advantages.
\blue{Compared to preliminary trial of using Thompson Sampling for dueling bandits, e.g., RCS \cite{Zoghi2014WSDM:RCS}, our D-TS algorithm has both practical and theoretical advantages.}

First, the double sampling structure of D-TS better suits   the nature of dueling bandits. Launching two independent rounds of sampling provides us the opportunity to select the same arm in both rounds and thus to compare the winners against themselves. Therefore, this double sampling structure leads to more extensive utilization of TS (e.g., compared to  RCS), and significantly reduces the regret. Moreover, this simple framework applies to general Copeland dueling bandits and achieves much better performance than existing algorithms such as CCB \cite{Zoghi2015NIPS:CDB}.
%One may suggest treating each pair of arms as a complex action and apply the simple framework of Thompson Sampling in \cite{Gopalan2014ICML:TS}. However, as discussed previously, not all comparisons provide information and it is unclear how to select the pair according to the samples, especially for general Copeland dueling bandits.
%Without special treatment, using the simple framework may get stuck on comparing non-winners.

Second,  leveraging the properties of this double sampling structure, we are able to obtain theoretical bounds for the regret of D-TS.  As noted in traditional MAB literature \cite{Agrawal2012COLT:TS,Agrawal2013AISTATS:TS2}, theoretical analysis of TS is usually more difficult than UCB-type algorithms.
The analysis in dueling bandits is even more challenging because the selection of arms involves more factors and the two selected arms may be correlated.
%For example, an arm that is selected as the first candidate may also have a higher probability (than that in traditional MAB) to be chosen as the second candidate.
To address this issue, our D-TS algorithm  draws  the two sets of samples independently.
Because their distributions are fully captured by historic comparison results,  when the first candidate is fixed, the comparison between it and all other arms is similar to traditional MAB and thus we can borrow the ideas for traditional MAB.  Using the properties of TS and confidence bounds, we show that  D-TS achieves $O(K^2 \log T)$ regret
for a general $K$-armed Copeland dueling bandit. More interestingly, the property that the sample distribution only depends on historic comparing results (but not $t$)  enables us to refine the regret using  a \emph{back substitution} argument, where we show that D-TS achieves $O(K \log T + K^2 \log \log T)$ in many practical scenarios and Condorcet dueling bandits.
%we have shown that we can bound the number of time-slots when a non-winner arm is chosen as the first candidate  by $O(\log T)$. Then by viewing the comparison between it and all other arms as a traditional MAB, we can bound the number of comparison between this arm and the suboptimal arms (that is beaten by it) is further reduced to $O(\log \log T)$ due to the concavity of the logarithmic function. Then the total regret is reduced to $O(K L_C \log T + K^2 \log \log T)$ regret, where $L_C$ is the number of arms that beats the Copeland winners.

Based on the analysis, we further refine the tie-breaking criterion in D-TS and propose its enhancement called D-TS$^+$. D-TS$^+$ achieves the same theoretical regret bound as D-TS, but performs better in practice especially when there are multiple winners.

% Furthermore, this algorithm applies to many dueling bandit problems with different definitions of winner, including both  the Condorcet winner \cite{Yue2012JCSS:DuelingBandits,Yue2009ICML:DuelingBandits}  and the Copeland winner \cite{Zoghi2015NIPS:CDB}.

In summary, the main contributions of this paper are as follows:
\begin{itemize}
\item We propose a D-TS algorithm and its enhancement D-TS$^+$ for general Copeland dueling bandits. The double sampling structure suits the nature of dueling bandits and leads to more extensive usage of TS, which significantly reduces the regret.
    %Our study also demonstrates how to deal with the unique difficulties when using Thompson Sampling in dueling bandits, e.g., using RUCB/RLCB-based elimination to avoid trapping in suboptimal comparisons.
\item We obtain theoretical regret bounds for D-TS. For general Copeland dueling bandits, we show that the proposed D-TS and D-TS$^+$ algorithms achieve $O(K^2 \log T)$ regret. In Condorcet dueling bandits and most practical scenarios, we further refine the regret bound to $O(K \log T + K^2 \log \log T)$ using a back substitution argument.
\item We evaluate the D-TS and D-TS$^+$ algorithms through experiments based on both synthetic and real-world data. The experiment results demonstrate the effectiveness of this double sampling structure.
\end{itemize}
\aftersec
\aftersec
\section{Related Work}
\aftersec
Many algorithms have been proposed to solve dueling bandits since \cite{Yue2012JCSS:DuelingBandits}. Earlier algorithms such as IF \cite{Yue2012JCSS:DuelingBandits}, BTM \cite{Yue2011ICML:BTM}, and SAVAGE \cite{Urvoy2013ICML:SAVAGE} belong to the ``explore-then-exploit'' family and only apply to  finite-horizon settings. For infinite horizon settings, recent work has generalized the traditional UCB and MED algorithms to dueling bandits. For example, RUCB \cite{Zoghi2014ICML:RUCB} and CCB \cite{Zoghi2015NIPS:CDB} are generalizations of UCB for Condorcet and general Copeland dueling bandits, respectively. \cite{Ailon2014ICML:UBDB} reduces dueling bandits to traditional MAB, which is then solved by their proposed UCB-type algorithms, MutiSBM and Sparring.
%\cite{Zoghi2014ICML:RUCB} extends the classic Upper Confidence Bound (UCB) method \cite{Auer2002ML:UCB} to dueling bandits and proposes a Relative Upper Confidence Bound (RUCB) algorithm that achieves $O(K \log T)$ regret in $K$-armed dueling bandits. The more recent work  \cite{Komiyama2015COLT:DB} proposes  a Relative Minimum Empirical Divergence (RMED) algorithm, which is shown to be optimal in the sense of both the asymptotic order $O(K \log T)$ and the constant coefficient, under the Condorcet assumption.
%These algorithms are proposed for Condorcet dueling bandits, while the existence of a Condorcet winner is not guaranteed in practice \cite{Urvoy2013ICML:SAVAGE,Zoghi2015NIPS:CDB}.
On the other hand, \cite{Komiyama2015COLT:DB} and the recently accepted work \cite{Komiyama2016ICML:CWRMED} extend the traditional MED algorithm to dueling bandits, where they present the lower bound of the regret and propose the corresponding optimal algorithms, including RMED \cite{Komiyama2015COLT:DB} for Condorcet dueling bandits, CW-RMED  and its computationally efficient version ECW-RMED \cite{Komiyama2016ICML:CWRMED} for general Copeland dueling bandits. Different from these existing work, we study algorithms for dueling bandits from the perspective of Thompson Sampling, which is expected to achieve lower regret in practice and more robust.
%Another definition of winner is the Borda winner, which is that arm that has the highest total probability of beating other arms. Because Borda dueling bandits can be reduced to the traditional MAB problem \cite{Urvoy2013ICML:SAVAGE,Zoghi2014ICML:RUCB}, only a few researchers study this problem with special structures, such as sparseness \cite{Jamieson2015AISTAT:SDB}. By treating each pair as an action, the SAVAGE algorithm \cite{Urvoy2013ICML:SAVAGE} applies to dueling bandits with all the above three definitions of winners, but it is an ``explore-then-exploit'' algorithm and exploring all pairs of arms may result in a large regret.


Dating back to 1933, Thompson Sampling \cite{Thompson1933FirstMAB} is one of the earliest algorithms for exploration/exploitation tradeoff and has been widely applied in traditional MAB.
%The Thompson Sampling algorithm makes decisions according to random samples drawn from the posterior distribution and updates the posterior distribution according to the system feedback under the taken action.
Empirical studies have shown that Thompson Sampling achieves performance better than or close to that of  UCB-type algorithms in practice \cite{Chapelle2011NIPS:TS}. However, theoretical analysis of Thompson Sampling is much more difficult  and a lot of efforts have been made to bound the regret theoretically.  In particular, \cite{Agrawal2012COLT:TS} proposes a logarithmic bound for the standard frequentist expected regret, whose constant factor is further improved in \cite{Agrawal2013AISTATS:TS2}.  On the other hand, through information-theoretic analysis, \cite{Russo2014TR:TS,Russo2014MOR:TS} derive the bounds for its Bayesian expected regret. Nowadays, Thompson Sampling becomes a popular method that has been applied in many variants of MAB \cite{Komiyama2015ICML:MP_TS,Qin&Liu2015IJCAI:TS,Gopalan2014ICML:TS} and other more complex problems, e.g., \cite{Gopalan2015COLT:TSMDP}.

Thompson Sampling has been preliminarily studied for dueling bandits. A rough idea was first discussed at a workshop \cite{Welsh2012LSOLDM:TS}, where the presenter suggests viewing the (normalized) preference matrix as the transition probability matrix for a Markov chain and selecting the arms by sampling from the posterior stationary distribution. Neither the formal description of this idea nor its theoretical analysis is available.
A recent work \cite{Zoghi2014WSDM:RCS} proposes a Relative Confidence Sampling (RCS) algorithm that combines Thompson Sampling with RUCB \cite{Zoghi2014ICML:RUCB}  for Condorcet dueling bandits. Under RCS, the first arm is selected by Thompson Sampling while the second arm is selected according to their RUCB. Empirical studies demonstrate the performance improvement by using RCS in practice, but no theoretical bounds on the regret are provided.


